Probabilistic data flow analysis: a linear equational approach

Speculative optimisation relies on the estimation of the probabilities that certain properties of the control flow are fulfilled. Concrete or estimated branch probabilities can be used for searching and constructing advantageous speculative and bookkeeping transformations. We present a probabilistic extension of the classical equational approach to data-flow analysis that can be used to this purpose. More precisely, we show how the probabilistic information introduced in a control flow graph by branch prediction can be used to extract a system of linear equations from a program and present a method for calculating correct (numerical) solutions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{150}
\providecommand{\publicationstatus}{Gabriele Puppis, Tiziano Villa (Eds.): Fourth International\\ Symposium on Games, Automata, Logics and Formal Verification\\
EPTCS 119, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.119.14}{10.4204/EPTCS.119.14}}

